Online Continual Learning for Anomaly Detection in IoT under Data Distribution Shifts

In this work, we present OCLADS, a novel communication framework with continual learning (CL) for Internet of Things (IoT) anomaly detection (AD) when operating in non-stationary environments. As the statistical properties of the observed data change with time, the on-device inference model becomes obsolete, which necessitates strategic model updating. OCLADS keeps track of data distribution shifts to timely update the on-device IoT AD model. To do so, OCLADS introduces two mechanisms during the interaction between the resource-constrained IoT device and an edge server (ES): i) an intelligent sample selection mechanism at the device for data transmission, and ii) a distribution-shift detection mechanism at the ES for model updating. Experimental results with TinyML demonstrate that our proposed framework achieves high inference accuracy while realizing a significantly smaller number of model updates compared to the baseline schemes.

==> tinyml/acronyms.tex <==
%a
\newacronym{ae}{AE}{autoencoder}
\newacronym{ap}{AP}{access point}
\newacronym{ad}{AD}{anomaly detection}
%b


%c
\newacronym{cl}{CL}{continual Learning}


%d
\newacronym{dnn}{DNN}{Deep Neural Network}
%e
\newacronym{en}{EN}{easy negative}
\newacronym{es}{ES}{edge server}
%f
\newacronym{fd}{FD}{fault detection}
\newacronym{fp}{FP}{false positive}
\newacronym{fpr}{FPR}{false positive rate}
\newacronym{fn}{FN}{False Negative}
%g

%h
\newacronym{hn}{HN}{hard negative}

%i
\newacronym{iot}{IoT}{Internet of Things}
\newacronym{iid}{i.i.d.}{independent and identically distributed}

%j 

%k
\newacronym{kpi}{KPI}{key performance indicator}
%m
\newacronym{mcu}{MCU}{micro controller unit}
\newacronym{ml}{ML}{machine learning}


%o
\newacronym{ocl}{OCL}{Online Continual Learning}
\newacronym{ocsvm}{OCSVM}{One-Class SVM}
%t
\newacronym{tinyml}{TinyML}{Tiny Machine Learning}
\newacronym{tp}{TP}{true positive}
\newacronym{tpr}{TPR}{true positive rate}


\newacronym{tdr}{TDR}{true (false) discovery rate}





==> tinyml/figures_tex/legend.tex <==
% \begin{tikzpicture}[inner sep=0pt, outer sep=0pt]

% \definecolor{darkgray176}{RGB}{176,176,176}
% \definecolor{darkturquoise0191191}{RGB}{0,191,191}
% \definecolor{green01270}{RGB}{0,127,0}
% \definecolor{lightgray204}{RGB}{204,204,204}
% \definecolor{steelblue31119180}{RGB}{31,119,180}

% \begin{axis}[
% legend cell align={left},
% legend style={
%   fill opacity=0.8,
%   draw opacity=1,
%   text opacity=1,
%   % at={(0.03,0.97)},
%   % anchor=north west,
%   draw=lightgray204
% },
% tick align=outside,
% tick pos=left,
% x grid style={darkgray176},
% xlabel={\(\displaystyle \mathbf{x}\)},
% xmin=-0.495, xmax=10.395,
% xtick style={color=black},
% y grid style={darkgray176},
% ylabel={\(\displaystyle \mathbf{v(x)}\)},
% ymin=-0.0891695609778769, ymax=1.87256078053542,
% ytick style={color=black},
% ]

% \addlegendentry{All-update}
% \addlegendentry{Random-update}
% \addlegendentry{Oracle OCLADS}
% \addlegendentry{OCLADS}
% \addlegendentry{No-update}
% \end{axis}

% \end{tikzpicture}

\begin{tikzpicture}[inner sep=0pt, outer sep=0pt]

% \definecolor{steelblue31119180}{RGB}{31,119,180}
% \definecolor{darkturquoise0191191}{RGB}{0,191,191}
% \definecolor{green01270}{RGB}{0,127,0}
% \definecolor{lightgray204}{RGB}{204,204,204}
% \definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkturquoise0191191}{RGB}{0,191,191}
\definecolor{green01270}{RGB}{0,127,0}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
    hide axis,
    legend cell align={left},
    legend style={
        fill opacity=0.8,
        draw opacity=1,
        text opacity=1,
        draw=lightgray204
    },
    legend columns=3
]

% Dummy invisible plots
\addplot[blue, thick] coordinates {(0,0)};
\addlegendentry{All-update}

\addplot[orange, thick] coordinates {(0,0)};
\addlegendentry{Random-update}

\addplot[red, thick] coordinates {(0,0)};
\addlegendentry{Oracle OCLADS}

\addplot[green01270, thick] coordinates {(0,0)};
\addlegendentry{OCLADS}

\addplot[steelblue31119180, thick] coordinates {(0,0)};
\addlegendentry{No-update}

\end{axis}
\end{tikzpicture}

